The Fishyscapes Benchmark: Measuring Blind Spots in Semantic Segmentation

Deep learning has enabled impressive progress in the accuracy of semantic segmentation. Yet, the ability to estimate uncertainty and detect failure is key for safety-critical applications like autonomous driving. Existing uncertainty estimates have mostly been evaluated on simple tasks, and it is unclear whether these methods generalize to more complex scenarios. We present Fishyscapes, the first public benchmark for uncertainty estimation in a real-world task of semantic segmentation for urban driving. It evaluates pixel-wise uncertainty estimates towards the detection of anomalous objects in front of the vehicle. We~adapt state-of-the-art methods to recent semantic segmentation models and compare approaches based on softmax confidence, Bayesian learning, and embedding density. Our results show that anomaly detection is far from solved even for ordinary situations, while our benchmark allows measuring advancements beyond the state-of-the-art.

==> embeddings.tex <==
\begin{figure*}[t!]
\centering
\def\iwidth{.25\linewidth}

\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{plots/lion_small.jpg}
\end{minipage}%
\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{plots/embeddings/fsdyn2_27_nll.jpg}
\end{minipage}%
\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{plots/embeddings/fsdyn2_27_tsne-mask.pdf}
\end{minipage}%
\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{plots/embeddings/fsdyn2_27_tsne-nll.pdf}
\end{minipage}

\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{plots/qualitative_small/fsdyn2_81_rgb.jpg}
\end{minipage}%
\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.98\linewidth]{plots/embeddings/fsdyn2_81_nll.jpg}
\end{minipage}%
\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{plots/embeddings/fsdyn2_81_tsne-mask.pdf}
\end{minipage}%
\begin{minipage}{\iwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{plots/embeddings/fsdyn2_81_tsne-nll.pdf}
\end{minipage}

\vspace{2mm}
\caption{\textbf{Visualization of the embeddings of a DeepLab layer.} From left to right, we show (a) the input image, (b) the pixel-wise NLL predicted by the normalizing flow, (c) the embeddings colored in blue (red) when associated with \ac{id} (\ac{ood}) pixels, and (d) the embeddings colored by predicted NLL with the jet colormap (red means high NLL). The first row shows a successful \ac{ood} detection, and the second row a failure case.}
\label{fig:embeddings}
%\vspace{-5mm}
\end{figure*}

==> method_overview.tex <==
\begin{figure*}[htb!]
\centering
\def\iwidth{.25\linewidth}

\begin{tikzpicture}
\node[inner sep=0pt, label=\scriptsize{Input}] at (0,0)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_rgb.jpg}};
\node[inner sep=0pt, label=\scriptsize{Softmax Entropy}] () at (.25\linewidth,0)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_entropy.jpg}};
\node[inner sep=0pt, label=\scriptsize{Dropout MI}] () at (.5\linewidth,0)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_mi.jpg}};
\node[inner sep=0pt, label=\scriptsize{Dirichlet Entropy}] () at (.75\linewidth,0)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_dir.jpg}};
    
\node[inner sep=0pt, label=below:\scriptsize{DeepLabv3+ Prediction}] at (0,-2.07)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_pred.png}};
\node[inner sep=0pt, label=below:\scriptsize{kNN Embedding Density}] at (.25\linewidth,-2.07)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_knn.jpg}};
\node[inner sep=0pt, label=below:\scriptsize{Learned Embedding Density}] at (.5\linewidth,-2.07)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_nll.jpg}};
\node[inner sep=0pt, label=below:\scriptsize{Void Classifier}] at (.75\linewidth,-2.07)
    {\includegraphics[width=\iwidth]{plots/qualitative_small/fs8_21_void}};
\end{tikzpicture}
\caption{\textbf{Example of out-of-distribution (OoD) detection:} We evaluate the ability of Bayesian (top) and non-Bayesian (bottom) methods to segment OoD objects (here a dog) based on a semantic segmentation model. Better methods should assign a high score (dark) to pixels belonging to the object only, and a low score (white) to in-distribution (background) pixels. The semantic prediction is not sufficient.}
\label{fig:overview}
\vspace{-3mm}
\end{figure*}
